GPG: A Simple and Strong Reinforcement Learning Baseline for Model Reasoning

Reinforcement Learning (RL) can directly enhance the reasoning capabilities of large language models without extensive reliance on Supervised Fine-Tuning (SFT). In this work, we revisit the traditional Policy Gradient (PG) mechanism and propose a minimalist RL approach termed Group Policy Gradient (GPG). Unlike conventional methods, GPG directly optimize the original RL objective, thus obviating the need for surrogate loss functions. By eliminating the critic and reference models, avoiding KL divergence constraints, and addressing the advantage and gradient estimation bias, our approach significantly simplifies the training process compared to Group Relative Policy Optimization (GRPO). Our approach achieves superior performance without relying on auxiliary techniques or adjustments. As illustrated in Figure 1, extensive experiments demonstrate that our method not only reduces computational costs but also consistently outperforms GRPO across various unimodal and multimodal tasks. Our code is available at https://github.com/AMAP-ML/GPG.

==> ICLR26/iclr_rebuttal_code_result_tab.tex <==
\begin{table}[htbp]
\centering
\caption{EvalPlus Code Result}
\label{tab:evalplus_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cc|cc|}
\hline
\multirow{2}{*}{\textbf{model}} & \multicolumn{2}{c|}{\textbf{HumanEval}} & \multicolumn{2}{c|}{\textbf{MBPP}} \\
\cline{2-5}
 & Base & Plus & Base & Plus \\
\hline
% deepseek-ai/DeepSeek-R1-Distill-Qwen-1.5B & 40.24\% & 37.20\% & 25.13\% & 22.49\% \\
GRPO & 38.41\% & 34.76\% & 24.60\% & 21.96\% \\
GPG & 37.80\% & 34.15\% & 26.19\% & 23.81\% \\
\hline
\end{tabular}
}
\end{table}


==> ICLR26/iclr_rebuttal_qa_result_tab.tex <==
\begin{table}[htbp]
\centering
\caption{Zero Shot evaluation results based on Light-eval. }
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|cccc|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Seed} & \multicolumn{4}{c|}{arc\string:challenge} & \multicolumn{4}{c|}{arc\string:easy} & \multicolumn{4}{c|}{hellaswag} & \multicolumn{4}{c|}{truthfulqa\string:mc} \\
 &  & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & mc1 & mc1\_stderr & mc2 & mc2\_stderr \\
\hline
% \multirow{4}{*}{DeepSeek-R1-Distill-Qwen-1.5B} & 0 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 1 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 2 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 3 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
% \hline
\multirow{4}{*}{GRPO} & 0 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 1 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 2 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 3 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
\hline
\multirow{4}{*}{GPG} & 0 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 1 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 2 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 3 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
\hline
\end{tabular}
}% end resizebox
\end{table}

==> ICLR26/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR26/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
% \setcitestyle{numbers,square}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multicol}
\usepackage{array}
% \usepackage{natbib}
\usepackage{algorithm, algorithmic}
\usepackage{enumitem}
\usepackage{tcolorbox}
\tcbuselibrary{most}
\tcbuselibrary{skins}
\usepackage{caption}
\usepackage{makecell}
\usepackage{pifont}
\usepackage{adjustbox}
\usepackage{amsfonts, amsmath, amsthm, graphicx, color, tikz, booktabs, multirow, bm, cases, mathtools, mathrsfs, pgfplots, subcaption, csvsimple}
\definecolor{iccvblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,allcolors=iccvblue]{hyperref}


\definecolor{mygray}{rgb}{0.9, 0.9, 0.9}
\definecolor{tcuserbg}{RGB}{245, 245, 245}
\definecolor{tcuserborder}{RGB}{210, 229, 255}
\definecolor{tcuserfont}{RGB}{0, 0, 0}
\definecolor{ForestGreen}{rgb}{0, 0.69, 0.31}
\definecolor{NavyBlue}{rgb}{0, 0.44, 0.75}

\newcommand{\hgreen}[1]{\textcolor{ForestGreen}{\textbf{#1}}} % highlight color
\newcommand{\hblue}[1]{\textcolor{NavyBlue}{\textbf{#1}}} % highlight color

\newcommand{\bop}[1]{\noindent\textbf{#1}}
\newcommand{\warn}[2]{~\textcolor{red}{@#1}~\textbf{\textit{#2}}~}
\newcommand{\ours}[0]{GPG}



\tcbset{
  enhanced,
  boxrule=1pt,
  colback=tcuserbg,
  colframe=tcuserborder,
  fonttitle=\bfseries,
  coltitle=tcuserfont,
  boxsep=5pt,
  arc=5pt,
  outer arc=5pt,
  left=10pt,
  right=10pt,
  top=2pt,
  bottom=2pt,
  attach boxed title to top left={yshift=-0.25\baselineskip-1mm,xshift=2mm},
  boxed title style={
    colback=tcuserborder,
    sharp corners,
    rounded corners=northeast,
    arc=3pt,
    outer arc=3pt,
    boxrule=0pt,
    boxsep=2pt,
  },
}

==> ICLR26/sec/0_abstract.tex <==
\begin{abstract}
Reinforcement Learning (RL) can directly enhance the reasoning capabilities of large language models without extensive reliance on Supervised Fine-Tuning (SFT). In this work, we revisit the traditional Policy Gradient (PG) mechanism and propose a minimalist RL approach termed Group Policy Gradient (GPG). Unlike conventional methods, GPG directly optimizes the original RL objective, thus obviating the need for surrogate loss functions. By eliminating the critic and reference models, avoiding KL divergence constraints, and addressing the advantage and gradient estimation bias, our approach significantly simplifies the training process compared to Group Relative Policy Optimization (GRPO). Our approach achieves superior performance without relying on auxiliary techniques or adjustments. As illustrated in Figure~\ref{fig:fig0}, extensive experiments demonstrate that our method not only reduces computational costs but also consistently outperforms GRPO across various unimodal and multimodal tasks.
% Our code is available at \url{https://github.com/AMAP-ML/GPG}.

\end{abstract}

==> ICLR26/sec/1_intro.tex <==
\section{Introduction}
\input{suppl/figure0}

Large Language Models (LLMs) have achieved substantial advancements, progressively narrowing the gap towards achieving Artificial General Intelligence (AGI)~\citep{o1,Deepseek-r1,bai2025qwen2,Deepseek-vl2,yao2024minicpm}. Recently, LLMs, exemplified by OpenAI o1~\citep{o1} and DeepSeek R1~\citep{Deepseek-r1}, adopt a strategy of generating intermediate reasoning steps before producing final answers. This approach markedly improves their efficacy in domain-specific tasks, such as mathematical reasoning~\citep{Numinamath,Omni-math,LISA,AIME24,Olympicarena}. The remarkable success of this technology is mainly attributed to the Reinforcement Fine-Tuning (RFT) method~\citep{schulman2017proximal,shao2024deepseekmath,DAPO-bytedance,ReMax,REINFORCE++,dai2026harder,ji2025tree,li2025adacurl,xiong2025hs}. Through the application of RFT, the models allocate additional time to ``deliberate'' prior to generating answers, thereby constructing intricate reasoning chains and subsequently enhancing overall model performance.

In contrast to Supervised Fine-Tuning (SFT), which involves training models on fixed input-output pairs to mimic correct responses, RFT introduces an iterative process that incentivizes models to generate coherent and logically structured reasoning paths. RFT leverages RL techniques, such as Proximal Policy Optimization (PPO) \citep{schulman2017proximal} and GRPO \citep{shao2024deepseekmath} to optimize decision-making during the generation of intermediate steps. Specifically, PPO ensures stability by constraining policy updates, preventing new strategies that deviate significantly from established behaviours. In contrast, GRPO enhances this process by evaluating performance across groups of actions, encouraging consistent improvements in reasoning quality. This dynamic and feedback-driven approach enables models to think more deeply, resulting in nuanced answers that better handle complex reasoning tasks compared to the more rigid and label-dependent training of SFT.



Despite the significant success of PPO in enhancing reasoning quality, it still suffers severely from the enormous resource consumption required during training. PPO necessitates the development and integration of both a critic model and a reference model, which not only complicates the training process but also substantially increases computational demands. 
Consequently, there is a growing trend toward simplifying the PPO method. For instance, ReMax~\citep{ReMax} removes the critic model by introducing a baseline value, which reduces the training GPU memory usage and accelerates the training process. Besides, GRPO eliminates the need for a critic model and utilizes normalized rewards within a sample group. 
% Furthermore, DAPO~\cite{DAPO-bytedance} removes the KL Divergence from GRPO and enhances the algorithm by introducing multiple technologies such as ``clip-higher'' and ``dynamic sampling''. Additionally, REINFORCE++~\cite{REINFORCE++} incorporates key optimization strategies from PPO while discarding the critic network, thus simplifying the training process and improving stability.

In addition to these methods to improve efficiency and stability, a very recent and concurrent work Dr. GRPO~\citep{liu2025understanding} studies the details of reward and loss normalization and states GRPO tends to generate more tokens. However, although it reveals the reward bias in the advantage function, we observe that its performance did not significantly outperform GRPO.

% A thorough examination of the evolution within the Reinforcement Learning (RL) community reveals that the widely adopted PPO algorithm essentially functions as a conservative surrogate for the original RL problem \citep{schulman2017proximal}. All existing enhancements to PPO continue to focus on optimizing the surrogate loss function. Consequently, two fundamental questions remain unresolved:
% % All improvements upon it are still optimizing the surrogate loss function
% \begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
%     \item  Is it feasible to transcend this intermediate strategy and directly optimize the original problem? 
%     \item If this is achievable, to what extent can the learning strategy be streamlined? 
% \end{itemize}

Let's review the birth of PPO. PPO was proposed as a general RL algorithm, with Atari games as primary evaluation benchmarks, where the policy network typically learns both visual representations and the control policy. In the LLM era, however, the policy is an LLM that already possesses strong representations from pretraining and SFT. Removing unnecessary components is important for scalability, which motivates rethinking simplified RL methods. Notably, PPO itself is a simplification of TRPO \citep{schulman2015trust}, which in turn builds on the policy-gradient algorithm. A major weakness of policy gradients is high variance, which can be mitigated by (i) using a value-function baseline in advantage estimation and (ii) sampling more trajectories—both common practices in the post-training training for LLMs. Thus, it is natural to build a streamlined method for reasoning.

In summary, our key contributions are as follows: 
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
\item We revisit the design of policy gradient algorithms \citep{sutton1998reinforcement} and propose a simple RL method that retains minimal RL components. Unlike conventional approaches, our method directly optimizes the objective function rather than relying on surrogate loss.

\item Our approach eschews the necessity for both a critic model and a reference model. Moreover, it imposes no distributional constraints. These characteristics confer substantial advantages for potential scalability.

\item We analyze and demonstrate the reward bias inherent in existing advantage functions and reveal the limitations of simplistic debiasing methods. Our exploration of the gradient estimate bias phenomenon has led us to propose a simple yet accurate gradient estimation (AGE) technique. To mitigate the potential issue of large variance in gradient estimation when the proportion of valid samples is excessively small, we introduce a simple thresholding mechanism to ensure a minimal partition of valid samples is maintained, followed by resampling.


% \item Extensive experiments demonstrated that GPG achieves superior performance than GRPO across various unimodal and multimodal visual tasks, while significantly reducing computational costs. 

\item Extensive experiments demonstrate that GPG achieves SOTA results across various unimodal and multimodal visual tasks.

\end{itemize}


==> ICLR26/sec/2_related.tex <==
\section{Related Work}
\textbf{Large Model Reasoning.}
Recent advancements in both LLM and Multimodal Large Language Model (MLLM) increasingly focus on enabling models to simulate human-like, stepwise reasoning processes. In the field of LLMs, researchers have pioneered methods such as Chain-of-Thought (CoT) prompting~\citep{o1,wei2022chain,kojima2022large,ye2025limoreasoning}, Tree-of-Thought~\citep{yao2023tree}, Monte Carlo Tree Search~\citep{feng2024alphazeroliketreesearchguidelarge,DeepSeek-Prover-V1.5,AlphaGeometryTrinh2024}, and the construction of complex SFT datasets~\citep{s1-stts}, to enhance performance in reasoning tasks.
Notably, approaches such as DeepSeek-R1~\citep{Deepseek-r1} employ large-scale RL with format-specific and result-oriented reward functions, guiding LLMs toward self-emerging, human-like, complex CoT reasoning with significant performance improvements in challenging reasoning tasks.
Meanwhile, MLLMs convert inputs from various modalities into a unified LLM vocabulary representation space for processing and exhibit superior performance in vision understanding tasks~\citep{Deepseek-vl2,liu2023visual,internvl25,gemini}.
Building on advancements in LLM reasoning, the research community collectively applies the DeepSeek-R1 methodology to MLLMs to enhance their visual reasoning capabilities, yielding remarkable progress~\citep{zhang2025r1,Visual-RFT,R1-V,VisualThinker-R1-Zero,yuan2025video,ji2026thinking,wang2026urban,yuan2025autodrive}.


\textbf{Reinforcement Learning.}
RL has driven significant progress in sequential decision-making, with policy gradient methods being fundamental to optimizing stochastic policies. The REINFORCE algorithm~\citep{williams1992simple} establishes early principles for gradient-based policy updates in trajectory-driven tasks. However, its high variance poses challenges for scalability. To address this, subsequent research focus on stabilizing policy optimization processes. Trust Region Policy Optimization (TRPO)~\citep{schulman2015trust} introduces constrained updates via quadratic approximations to ensure monotonic improvement. This approach is further refined by PPO~\citep{schulman2017proximal}, which employed clipped objective functions to simplify the optimization process. Subsequent studies seek to enhance the PPO algorithm \citep{zheng2023secrets} or elaborate on its implementation \citep{engstrom2019implementation}. PPO achieves widespread use in language model alignment and robotic control. However, the algorithm's dependence on conservative policy updates or heuristic clipping thresholds can undermine its exploration potential in favour of stability, which poses a significant challenge in complex domains requiring dynamic strategy adaptation.

Limited by space, more related work is discussed in Section~\ref{sec:more_related work}.


==> ICLR26/sec/3_method.tex <==
\section{Method}
\subsection{Preliminary and Task Formulation}

RL is a computational approach to learning through interaction, where an agent seeks to maximize cumulative rewards by selecting optimal actions within an environment. The RL problem is typically defined by a policy $\pi_{\theta}$, which maps states to actions, and aims to optimize the expected return.  The core idea behind policy gradient methods is to use gradient ascent to iteratively adjust the policy parameters. The learning objective is maximizing the return   $\mathcal{J}(\theta)$,
\begin{equation}
\mathcal{J}(\theta) = \max_{\theta} \mathbb{E}_{\pi_{\theta}} \left[ \sum_{t=0}^{T} r_t \right].
\end{equation}


The policy gradient theorem \citep{sutton1998reinforcement} proves that the above problem can be converted into estimating the gradient,
\begin{equation}
\label{eq:pg}
\nabla_{\theta} \mathcal{J}(\theta) = \mathbb{E}_{\pi_{\theta}} \left[ \nabla_{\theta} \log \pi_{\theta}(a_t \mid s_t) Q^{\pi_{\theta}}(s_t, a_t) \right],
\end{equation}
where $Q^{\pi_{\theta}}(s_t, a_t)$ is the action-value function, representing the expected return when taking action $a_t$ in state $s_t$ and following policy $\pi_{\theta}$ thereafter.

To reduce the variance,  the advantage function $A^{\pi_{\theta}}(s_t, a_t)$ is often used, leading to the policy gradient update rule:
\begin{equation}
\nabla_{\theta} \mathcal{J}(\theta) = \mathbb{E}_{\pi_{\theta}} \left[ \nabla_{\theta} \log \pi_{\theta}(a_t \mid s_t) A^{\pi_{\theta}}(s_t, a_t) \right].
\end{equation}


\textit{One-step advantage estimation} can be mathematically formulated as \citep{sutton1998reinforcement}:
\begin{equation}
A^{\pi_{\theta}}(s_t, a_t) = Q^{\pi_{\theta}}(s_t, a_t) - V^{\pi_{\theta}}(s_t),
\label{eq: advantage}
\end{equation}
where $V^{\pi_{\theta}}(s_t)$ is a function of $s_t$. In principle, $V^{\pi_{\theta}}(s_t)$ can take any functional form. One commonly employed function is the value function, which represents the expected return when starting from state $s_t$ and following policy $\pi_{\theta}$.
While GAE~\citep{GAE} offers a more sophisticated approach to balance bias and variance in advantage estimation, we find that in the context of model reasoning, one-step estimation is sufficiently effective for achieving good performance. This simplicity is particularly advantageous in scenarios where computational efficiency is paramount.

Given a sequence of questions and instructions, the model is tasked with generating corresponding answers. Subsequently, rewards are returned based on predefined reward models or hand-crafted rules. Our objective is to leverage these reward signals to optimize our policy, thereby enhancing the model's ability to generate accurate and contextually appropriate responses.

However, designing or obtaining accurate rewards for intermediate steps is nontrivial \citep{Deepseek-r1}. To address this challenge, we simplify our problem as follows. Given a question and prompt $s$, we sample an action $a$ from policy $\pi_{\theta}$ and obtain a final reward signal $r$. Note that the policy distribution $\pi_{\theta}$
  is modeled in an autoregressive manner. In this setting, we can leverage policy gradient methods to optimize the policy.


\subsection{Group Policy Gradient}
Our proposed method, Group Policy Gradient (GPG), is designed to address the issue of high variance in policy gradient estimation in the absence of a value model. By leveraging group-level rewards, GPG stabilizes learning and enhances the robustness of reinforcement learning training. Specifically, GPG utilizes the mean reward within each group to normalize the rewards, thereby effectively reducing variance. This approach eliminates the need for a traditional value model, thereby simplifying the training process and enhancing computational efficiency. The name ``Group Policy Gradient'' reflects our method's core mechanism of utilizing group-level mean rewards to stabilize and optimize learning.

The core objective of GPG is defined as:
\begin{equation}
\begin{aligned}
\mathcal{J}_{\text{GPG}}(\theta) = & \, \mathbb{E}_{(q,a) \sim \mathcal{D}, \{o_i\}_{i=1}^{G}} 
& \left[
\frac{1}{\sum_{i=1}^{G}{|o_i|}} \sum_{i=1}^{G}  \sum_{t=1}^{|o_i|}
\left( - \log \pi_{\theta}(o_{i,t} \mid q, o_i,<t) \hat{A}_{i,t} \right)
\right] ,
\end{aligned}
\end{equation}
where $o_i$ represents the individual responses in the group $G$, and the advantage of the $i$-th response is calculated by normalizing the group-level rewards $\{R_i\}_{i=1}^{G}$:
\begin{equation}
\label{equ:advantages}
\hat{A}_{i,t} = \frac{r_i - \text{mean}(\{R_i\}_{i=1}^{G})}{{F_{norm}}}.
\end{equation}
% $F_{norm}$ is an \textbf{optional} kind of normalization，which is usually applied with reward cliping to avoid unexpected out-lier value \cite{mnih2016asynchronous,schulman2017proximal}. One common practice is standard variance within a training batch. 
$F_{norm}$  is an \textbf{optional} normalization technique, which is commonly applied in conjunction with reward clipping to mitigate the impact of unexpected outlier values. One widely adopted practice is to employ standard variance normalization within a training batch \citep{mnih2016asynchronous,schulman2017proximal}. This approach helps stabilize the training process by reducing the variance of the reward signal, which is particularly important when dealing with environments where the magnitude of rewards can vary significantly, such as in different Atari games. By normalizing the reward signal, the model becomes less sensitive to extreme values, thereby improving the robustness and convergence of the training algorithm. However, in the reasoning tasks involving large models, the reward is typically well-defined and does not suffer from the same variance issues observed in other environments. As for the Math reasoning problem, it is a common practice to award the right answer with 1.0 and the wrong answer with 0.0.
% In such scenarios, the introduction of $F_{norm}$ may not only be unnecessary but could also potentially introduce \textbf{reward bias} that deviates from the original problem formulation. 

We utilize a basic Math Reasoning setting \footnote{huggingface/open-r1/recipes/Qwen2.5-Math-7B/grpo/config\_simple\_rl.yaml} of SimpleRL from open-r1 \citep{open-r1}, using only the MATH-lighteval dataset to facilitate rapid experimental validation. Specifically, we remove the format reward and only enable the accuracy reward for simplicity.

\input{tab/open-r1}

The critical component: $\hat{A}_{i,t}$, has been underexplored in prior research in reasoning. This gap in the literature highlights the need for further investigation of the role and impact of $\hat{A}_{i,t}$ within reasoning tasks.  There are two unresolved problems.
% \begin{itemize}

\bop{The $\hat{A}_{i,t}$ should not introduce reward bias}. Otherwise, bias deviates from the original problem formulation. GRPO \citep{shao2024deepseekmath} formulates it as $F_{norm}=\operatorname{std}\{R(o)\}$, which is essentially a function of $s_t$ in Equation~\ref{eq:pg} and explicitly introduces the reward bias. Since we aim to solve the original problem, we don't want to apply a surrogate or bias.  However, As shown in Table~\ref{tab:open-r1}, if we remove this bias item,  i.e. $F_{norm}=1$, it (43.9\%) \textit{cannot clearly outperform} GRPO (43.7\%), which is opposite to the observation of a concurrent work Dr. GRPO \citep{liu2025understanding}. 

\bop{Examples of all right or wrong responses within a group introduce bias for the estimation of the gradient}. Given a training batch of batch size $B$, let the gradient of the $i$-th sample be denoted as $g_{i}$. Without loss of generality, assume that the first $M$ examples within the batch are all right or wrong responses within a group. The standard backpropagation (BP) algorithm estimates the gradient as: $\mathbf{g}=\frac{\sum^{B}_{i=1} \mathbf{g_i}}{B}=\frac{\sum^{B}_{i=M+1} \mathbf{g_i}}{B}$. However, the first $M$ examples are not valid for gradient estimation and contribute zero gradient. Therefore, the more accurate gradient estimation (AGE) can be written as:
\begin{equation}
\label{eq:alpha}
\mathbf{\hat{g}}=\frac{\sum^{B}_{i=M+1} \mathbf{g_i}}{B-M}=\mathbf{g}\frac{B}{B-M}=\alpha \mathbf{g}, \alpha = \frac{B}{B-M}.
\end{equation}
It should be noted that the value $\alpha$ is not a constant and it varies across different sample batches. We also illustrate $\alpha$ with different steps in Figure~\ref{fig:num_zero_one}, which indicates the necessity of gradient correction.
As for multi-GPU training, to achieve more accurate gradient calculations, it is advisable to gather all non-zero gradient samples across all GPUs and compute the average gradient uniformly. This approach can be implemented through a custom gradient aggregation function, which leads to increased communication overhead.
 Instead, we derive another equivalent format, which doesn't require extra cost, and we provide the proof in Section \ref{sec:gradient_error}. Therefore, given a batch sample, the objective can be written as
\begin{equation}
\label{eq: age_loss}
\begin{aligned}
\hat{\mathcal{J}}_{\text{GPG}}(\theta) = \alpha \mathcal{J}_{\text{GPG}}(\theta).
\end{aligned}
\end{equation}
As shown in Table~\ref{tab:open-r1}, our method achieves an average score of 47.8\%, being equipped with AGE. 
\input{suppl/num_zero_one}

In a scenario where we reject the $M$ examples and resample responses in a manner similar to the approach presented in a recent work \citep{DAPO-bytedance} until $M$ equals 0, $\alpha$ is set to 1. However, this particular setting is not training-efficient. The reason is that the training time is constrained by the worker that takes the longest to collect the desired examples. In contrast, our proposed method demonstrates superior efficiency. Moreover, it can automatically adjust the loss based on the performance of the sample batch.

We also evaluate a setting of reward normalization of GRPO, where $F_{norm}$=${\operatorname{std}\{R(o)\}}$,$\alpha$=1, and show the result in Table~\ref{tab:open-r1}. It outperforms $F_{norm}$=1,$\alpha$=1 by 1.4$\%$ average score. This motivates us to dive into the source of the improvement. We plot the std of the reward in Figure~\ref{fig:num_zero_one}. Note that the std is calculated by averaging the std of each group, whose value ranges from 0.10 to 0.35. And $\alpha$ varies from 1.5 to 4.0. The reward normalization of GRPO provides such a diving std (within a group) mechanism, which has some gradient correction effect. 


% \input{tab/open-r1}
% Therefore, when considering the application of any normalization technique, it is crucial to carefully evaluate its necessity and potential impact on the model's performance and the integrity of the task at hand.


%\text{std}(\{R_i\}_{i=1}^{G})
% % w/o std
% \begin{equation}
% \label{equ:advantages}
% \hat{A}_{i,t} = r_i - \text{mean}(\{R_i\}_{i=1}^{G}).
% \end{equation}

% This normalization technique plays a pivotal role in reducing variance by ensuring that individual rewards are considered in the context of group dynamics, thereby fostering more stable and efficient learning even without a value model. 

% The GPG approach demonstrates that leveraging structured reward systems can yield significant improvements in reinforcement learning performance, highlighting the potential for future developments that minimize dependency on traditional models while maintaining robust training efficacy.


\input{tab/compare}

\bop{Thresholding minimal partition of valid samples and resampling to reduce variance.} While our approach provides an unbiased estimation of the gradient, it may encounter issues with high variance when the proportion of valid samples is excessively low. To mitigate this, we introduce a threshold $\beta_{th}=\frac{1}{\alpha_{th}}$ for the proportion of valid samples. When this proportion falls below the given value, we accumulate the valid samples into the resampled subsequent batch until the proportion exceeds the threshold. This strategy effectively reduces the variance of the gradient estimation, thereby enhancing the stability and convergence rate of the model training process. It is worth noting that this strategy further improves the performance, as demonstrated in Table~\ref{tab:open-r1}.
% It is important to highlight that this strategy can further enhance the performance, as demonstrated in Table~\ref{tab:open-r1}.



RL algorithms vary significantly in their approaches to tackling variance and optimizing policies. Two key components in many RL algorithms are surrogate loss and policy constraints. We summarize the main comparisons among various frameworks in Table~\ref{tab:compare}. Our method stands out by preserving the simplest form, which not only ensures ease of implementation but also maintains high efficiency and effectiveness.
%


% Overall, GPG represents an innovative step forward, integrating the benefits of reward normalization to enhance learning efficiency and adaptability, setting the stage for future advances in reinforcement learning strategies that emphasize flexible exploration and learning dynamics.



==> ICLR26/sec/4_experiment.tex <==
\section{Experiments}
\label{sec:exp}
All experimental settings are meticulously controlled to ensure fair comparisons. We closely adhere to the hyperparameters employed by GRPO, despite their suboptimality for our approach. Notably, our method consistently outperforms GRPO across all tasks, achieving superior performance with clear margins. These results underscore the robustness and efficacy of our proposed method.


\subsection{Experimental Setup}
\label{Section3.1}
\bop{Dataset and Benchmarks.}
In the unimodal scenario, we utilize datasets from multiple sources such as open-s1, open-rs \citep{open-rs}, and MATH-lighteval \citep{hendrycks2021measuring} for training. Specifically, we train the DeepSeek-R1-Distill-Qwen-1.5B base model with the open-s1 dataset, resulting in the GPG-RS1 model. Similarly, training with the open-rs dataset produces the GPG-RS3 model. Furthermore, we perform ablation studies using the MATH-lighteval dataset on the Qwen2.5-Math-7B base model. To compare the overall performance on the 7B model, we utilize the dataset from \citep{DAPO-bytedance}, and the detailed setting is shown in Section~\ref{sec:detailed setting}.
% In order to make comparison with other recent work, we utilize the simplelr\_qwen\_level3to5 dateset \cite{zeng2025simplerl}.

These datasets encompass a wide range of problem types and difficulty levels. To assess the reasoning capabilities of the models, we employ five distinct mathematics-focused benchmark datasets: AIME24, MATH-500 \citep{AIME24,hendrycks2021measuring}, AMC23, Minerva \citep{lewkowycz2022solving}, and OlympiadBench \citep{Olympicarena}. 


In the multimodal case, we handle a variety of tasks. Specifically, for the visual reasoning task, we utilize approximately $12,000$ samples from the SAT dataset~\citep{SAT-Dataset} for training and perform evaluations on the CV-Bench dataset~\cite{CV-Bench}. In addressing the geometry reasoning task, by following R1-V~\citep{R1-V}, we train on around $8,000$ samples from the GEOQA training set~\citep{R1-V} and subsequently evaluating performance on the GEOQA test set~\citep{GEOQA}. For both the classification and reasoning grounding tasks, we follow Visual-RFT to conduct few-shot classification training on Flower102~\citep{Flower102}, Pets37~\citep{Pets37}, FGVCAircraft~\citep{FGVCAircraft}, Car196~\citep{Car196}, respectively. Additionally, training is conducted on $239$ samples from the LISA training set~\citep{LISA}. All evaluations are carried out using the corresponding test sets associated with these training sets.

\bop{Implementation Details.} 
Our approach is broadly applicable across a wide range of reinforcement learning tasks. To demonstrate its versatility and efficacy, we conduct experiments encompassing both unimodal and multimodal scenarios. These experiments are performed on NVIDIA H20 GPUs and NPUs from China. For each experiment, we adhere strictly to the implementation of original code base, ensuring consistent training and evaluation procedures. The implemented GPG method can refer to Algorithm~\ref{alg:GPG}, and more detailed settings can refer to Appendix~\ref{appendix:More-Implementation-Details}.
\input{suppl/gpg_algo}


% For mathematical reasoning task, we present the following system prompt examples~\cite{open-rs,open-r1}:
% \input{suppl/Prompt-for-openr1}



% \input{tab/open-rs-15B}
\input{tab/math-all-15B}
% \input{tab/open-r1}
\input{tab/math-all-7B}

\subsection{Unimodal Task Evaluation}
\label{sec:main-results}

% \subsubsection{Unimodal Task}
To evaluate our method, we select two models: a strong 1.5B distilled SFT model (DeepSeek-R1-Distill-Qwen-1.5B) and a 7B base model.

% Additionally, the performance of GPG are evaluated in comparison to GRPO~\cite{shao2024deepseekmath} using  Qwen2.5-Math-7B model,
% as detailed in Table~\ref{tab:open-r1}. Notably, the GPG settings \((F_{\text{norm}}\!=\!1, \alpha\!=\!1) \) and \((F_{\text{norm}}\!=\!\text{std}\{R(o)\}, \alpha\!=\!1) \) demonstrate clear advantages on OlympiadBench, outperforming both the standard GRPO and Dr. GRPO configurations. The most prominent GPG setting, \((F_{\text{norm}}\!=\!1, \alpha\!=\!\frac{B}{B-M}) \), achieves an average score of 47.8\%. This high score is attributed to the novel gradient estimation technique AGE, which corrects for reward biases across different sample batches. Besides, the parameter \(\alpha\) varies dynamically, adapting to the batch composition, thereby enhancing training efficiency and accuracy. The experiments conducted validate the method's superior generalization ability, providing substantial improvements over the baseline Qwen2.5-Math-7B model and other advanced configurations.

\bop{Mathematical Reasoning using 1.5B model (A strong SFT model).} Compared with other 1.5B distilled models, our models exhibit superior performance with average accuracy 55.7\% of GPG-RS1, as illustrated in Table~\ref{math-all-15B}. Additionally, GPG-RS1 and GPG-RS3 shows strong results in AMC23 with a score of 77.5\% and 80.0\%, obviously surpassing Open-RS 67.5\% and 70.0\%. Both GPG-RS1 and GPG-RS3 demonstrate competitive performance across various benchmarks, particularly excelling in MATH-500 with scores of 87.6\% and 85.0\%, and OlympiadBench with scores of 50.5\% and 52.4\%.
% We systematically evluate the performance of GPG across five benchmark datasets and show the result in  Table~\ref{tab:open-rs}. Compared to GRPO~\cite{shao2024deepseekmath}, our GPG approach exhibits a substantial performance enhancement, achieving an average improvement of 2.6\%. Overall, the GPG model attains an average accuracy of 55.7\%. Significant improvements over GRPO are evidenced in the MATH-500 and AMC23 benchmarks, showing accuracy improvements of 3.8\% and 10.0\%, respectively. These results highlight the effectiveness of GPG in enhancing mathematical reasoning capabilities.



% GPG achieves a higher average accuracy of 45.3\%, representing an improvement of 1.6\% than GRPO. This enhancement illustrates the improved reasoning capabilities provided by GPG, particularly notable in specific benchmarks such as AIME24 (+6.6\%) and OlympiadBench~\cite{Olympicarena} (+3.6\%). Moreover, GPG achieves an average improvement of 2.6\% over Dr.~GRPO, demonstrating significant enhancements with a 10.0\% increase on AMC23 and a 2.0\% gain on OlympiadBench~\cite{Olympicarena}.
% These advancements highlight the utility of GPG in RL training for critical mathematical reasoning tasks.
\bop{Mathematical Reasoning using 7B model.} As illustrated in Table~\ref{math-all-7B}, GPG-7B achieves an average score of 57.7\% and outperforms other baselines with clear margins. This exceptional performance is further highlighted in the AMC23 and Minerva, where GPG-7B attained a leading score of 82.5\% and 39.0\%, exceeding SimpleRL-Zero-7B by impressive margins of 22.3\% and 11.4\%, respectively. Moreover, GPG-7B consistently exhibits superiority across most benchmarks, outperforming the recent state-of-the-art method, Oat-Zero-7B, by an average of 6.3\%.
% \input{tab/VisualThinker-R1-Zero-CV-Bench}
% \input{tab/GEOQA-LISA-merge}
% \input{tab/Visual-RFT-CLS}
\input{tab/mllm_tab_all}
\subsection{Multimodal Task Evalutaion}

We further evaluate our method on several very recent multimodal benchmarks, most of which report results based on GRPO.


\bop{Geometry Reasoning.}
In addition to visual reasoning, MLLMs exhibit notable proficiency in geometry reasoning. To evaluate the efficacy of the GPG method in this domain, we employ an experimental setup similar to that used in R1-V~\citep{R1-V} using the GEOQA~\citep{GEOQA} dataset. The results, presented in Table~\ref{tab:GEOQA}, indicate that the GPG method achieved a score of 51.33\%, surpassing the GRPO's score of 47.48\% by 3.85\% points. This demonstrates the superior performance of the GPG method in addressing complex geometric reasoning tasks.

\bop{Classification.}
Beyond the evaluation of reasoning tasks, we also assess the enhancement of the GPG method over GRPO in image perception tasks. As shown in Table~\ref{tab:CLS}, the GPG method achieves an average score of 89.0\% across four classification datasets, surpassing GRPO by 7.1\% points. Additionally, our method consistently produces improvements across all four classification datasets, underscoring its superiority in image perception tasks.

\bop{Visual Reasoning.}
We initially evaluate the GPG method using the CV-Bench~\citep{CV-Bench} visual reasoning dataset, strictly adhering to the parameter settings of VisualThinker-R1-Zero. As illustrated in Table~\ref{tab:CVBench}, the GPG method demonstrates a significant improvement in performance. Specifically, it attains a score of 76.15\% on CV-Bench, representing an increase of 16.68\% points compared to the 59.47\% score achieved by GRPO.

\bop{Reasoning Grounding.}
The final critical aspect of evaluating MLLMs involves precisely identifying objects according to user requirements. To this end, we employ the Qwen2-VL-2B model for grounding tasks using the LISA dataset~\citep{LISA}, with the results presented in Table~\ref{tab:LISA}. In comparison to the GRPO method, the GPG approach demonstrates a substantial enhancement, improving all metrics by over 14.0\% points. This significant improvement underscores the superiority of the GPG method in object localization, leading to considerable advancements in reasoning and perception capabilities.


% \input{suppl/15B_loss}
\subsection{Ablation Study and Discussion}
\bop{Case Study and Training Analysis.}
We present the reasoning processes of GPG and GRPO, as illustrated in Figure~\ref{fig:case} (supplementary). Compared to GRPO, the GPG approach demonstrates a more comprehensive and accurate reasoning capability, whereas GRPO exhibits errors in formula analysis. Consequently, GPG arrives at the correct solution, while GRPO produces an incorrect result. In Figure~\ref{fig:training_metrics}, we present a range of real-time training metrics to illustrate the effectiveness of GPG as a straightforward yet strong RL algorithm.

% \bop{Sensitivity on $\beta_{th}$}. 

\bop{Sensitivity on Group Size.} We study the effect of the number of generations within a group. As shown in Table~\ref{tab:ablation_ngen}, increasing the group size from 2 to 16 leads to progressive improvements across most metrics. Specifically, the Average performance improves steadily with larger group sizes. We choose 8 to achieve a good tradeoff between training cost and performance.


\bop{Comparison with Various RL Methods.}
We attempt to explain the differences between GPG and other RL methods in the simplest way. As shown in Table~\ref{tab:RL-method-Formula-Comparison}, it can be seen that the loss of GPG does not include the ``CLIP term'' and the ``KL divergence''. Its form and calculation are the simplest, and as discussed in Section~\ref{sec:main-results}, its performance is better than other methods.

\bop{Comparison with DAPO \citep{DAPO-bytedance}}.
We meticulously control the experimental settings and rigorously reported the results in Table~\ref{tab:ablation_dapo}. All models are trained on the same dataset and for the same number of steps (1100). 
In contrast to DAPO \citep{DAPO-bytedance}, which incorporates all proposed components, our method focuses exclusively on the accuracy reward. Despite this, our approach achieves superior performance with reduced training and data costs. DAPO, which constructs fully valid batches through dynamic sampling, often requires more batches and may waste valid samples in the final batch. In contrast, our method avoids these inefficiencies, ensuring optimal resource utilization and enhanced performance.
\input{tab/abaltion_dapo}

\bop{KL constraint.} 
In principle, our method is designed to optimize the original reinforcement learning (RL) problem directly. And it's a bit strange without imposing any distribution constraints. Despite this, we conduct an ablation study to evaluate the impact of adding a distribution constraint. The results are presented in Table~\ref{tab:ablation_std_norm}. Our findings indicate that incorporating such a constraint negatively impacts performance. 

Limited by space, we provide more ablation studies in Section~\ref{sec:more_ablations}.

\subsection{Impact and Limitation Discussion}
\label{sec:4_experiment:Broader_Impact}
Achieving advanced general intelligence critically depends on augmenting the reasoning capabilities of models, with efficient and scalable reinforcement learning methods serving as a cornerstone. Our proposed approach investigates a minimalist strategy that aims to enhance reasoning capacity through simplicity and efficiency, thereby potentially facilitating the development of scalable systems. However, given the constraints of our computational budget, we do not evaluate our method on extremely large models.


==> ICLR26/sec/5_conclusion.tex <==
\section{Conclusion}
In this paper, we introduce GPG, which effectively addresses the critical challenges inherent in reinforcement fine-tuning approaches such as PPO and GRPO. By directly incorporating group-based decision dynamics into the standard PG method, GPG simplifies the training process and significantly reduces computational overhead without sacrificing reasoning quality.  This breakthrough provides a more efficient framework for training advanced LLMs capable of complex reasoning, thereby contributing to more resource-effective and scalable artificial intelligence systems.

==> ICLR26/tab/GEOQA-LISA-merge.tex <==
\begin{table*}[!ht]
\begin{minipage}[ht]{0.44\textwidth}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.5cm}
% \captionsetup{skip=5pt}
\centering
\begin{tabular}{lc}
\toprule
Models & GEOQA$_{\text{Test}}$
\\
\midrule
Qwen2.5-VL-3B-Instruct & 35.41 \\
\midrule
~~$+$ GRPO & 47.48  \\
\rowcolor{mygray}~~$+$ GPG & 50.80  \\
% ~~$\Delta$ & \bf{+3.32} \\
\bottomrule
\end{tabular}
\caption{Geometry reasoning results on GEOQA~\cite{GEOQA}. GPG is better than GRPO.}
\label{tab:GEOQA}
\end{minipage}
\hfill
\begin{minipage}[ht]{0.52\textwidth}
\centering
\begin{tabular}{lccc}
\toprule
Models & mIoU$_{\text{test}}$ & mIoU$_{\text{val}}$ & gIoU$_{\text{test}}$
\\
\midrule
Qwen2-VL-2B & 26.9 & 30.1 & 25.3 \\
\midrule
~~$+$ SFT & 28.3 & 29.7 & 25.3 \\
~~$+$ GRPO & 37.6 & 34.4 & 34.4 \\
\rowcolor{mygray}~~$+$ GPG & 51.5 & 53.4 & 49.5 \\
% ~~$\Delta$ & \bf{+13.9} & \bf{+19.0} & \bf{+15.1}\\
\bottomrule
\end{tabular}
\caption{Reasoning grounding results on LISA~\cite{LISA}. GPG surpasses GRPO in reasoning grounding with 239 training images.}
\label{tab:LISA}
\end{minipage}
\end{table*}

==> ICLR26/tab/RL-method-Formula-Comparison.tex <==
\begin{table}[h]
\scriptsize
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.6mm}
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|c|c}
\toprule
\textbf{RL Method} &  \textbf{Loss Function} & \textbf{Advantage Function} \\
\midrule
PPO~\citep{schulman2017proximal} &
\makecell{$\begin{aligned}
\mathcal{L}_{\text{PPO}} = & - \min\left[\frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)} \cdot A,
\underbrace{\operatorname{clip}\left(\frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)}, 1-\epsilon, 1+\epsilon \right)}_{\text{CLIP}} \cdot A \right]
\end{aligned}$}
&
\makecell{
where $A$ computed by \\
applying GAE~\citep{GAE} based on \\
rewards and the \textbf{critic model}.
}
\\

GRPO~\citep{shao2024deepseekmath} &
\makecell{$\begin{aligned}
\mathcal{L}_{\text{GRPO}} = & -\left( \min \left[ \frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)} \cdot A, \text{CLIP} \cdot A \right] - \beta \mathbb{D}_{KL}\left[\pi_\theta \| \pi_{ref}\right] \right)
\end{aligned}$}
&
\makecell{$\begin{aligned}
A = & \frac{R(o)-\operatorname{mean}\{R(o)\}}{\operatorname{std}\{R(o)\}}
\end{aligned}$}
\\

Dr. GRPO~\citep{liu2025understanding} &
\makecell{$\begin{aligned}
\mathcal{L}_{\text{Dr.GRPO}} = \mathcal{L}_{\text{PPO}}
% & - \min \left[ \frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)} \cdot A, \text{CLIP} \cdot A \right]
\end{aligned}$}
&
\makecell{$\begin{aligned}
A = & R(o)-\operatorname{mean}\{R(o)\}
\end{aligned}$}
\\


DAPO~\citep{DAPO-bytedance} &
\makecell{$\begin{aligned}
\mathcal{L}_{\text{DAPO}} = & - \min \left[ \frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)} \cdot A, \operatorname{clip}\left(\frac{\pi_{\theta}(o)}{\pi_{\theta_{old}}(o)}, 1-\epsilon_{\text{low}}, 1+\epsilon_{\text{high}} \right) \cdot A \right]
\end{aligned}$}
&
\makecell{$\begin{aligned}
A = & \frac{R(o)-\operatorname{mean}\{R(o)\}}{\operatorname{std}\{R(o)\}}
\end{aligned}$}
\\

\textbf{GPG} &
\makecell{$\begin{aligned}
\mathcal{L}_{\text{GPG}} = & - \log \pi_{\theta}(o) \cdot A
\end{aligned}$}
&
\makecell{$\begin{aligned}
A = & \alpha * (R(o)-\operatorname{mean}\{R(o)\}) 
\end{aligned}$}
\\
\bottomrule
\end{tabular}
}
\caption{Comparison of various RL methods, we explain in the simplest form.}
\label{tab:RL-method-Formula-Comparison}
\end{table}

==> ICLR26/tab/Visual-RFT-CLS.tex <==
\begin{table}[!ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|c|cccc}
\toprule
Models & Average & Flower102~\cite{Flower102} & Pets37~\cite{Pets37} & FGVC~\cite{FGVCAircraft} & Cars196~\cite{Car196}
\\
\midrule
Qwen2-VL-2B  & 56.0 & 54.8 & 66.4 & 45.9 & 56.8 \\
\midrule
~~$+$ SFT & 55.6 & 58.5 & 55.5 & 67.9 & 40.5 \\
~~$+$ GRPO & 81.9 & 71.4 & 86.1 & 74.8 & 95.3 \\
\rowcolor{mygray}~~$+$ GPG & 86.0 & 73.0 & 87.1 & 86.8 & 97.1 \\
% ~~$\Delta$ & \bf{+4.1} & \bf{+1.6} & \bf{+1.0} & \bf{+12.0} & \bf{+1.8} \\
\bottomrule
\end{tabular}
\caption{4-shot Results on Four Fine-grained Classification Datasets. GPG shows consistently better results than GRPO on $4$ classification datasets.}
\label{tab:CLS}
\end{table}

==> ICLR26/tab/VisualThinker-R1-Zero-CV-Bench.tex <==
\begin{table}[!ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\begin{tabular}{l|c|cccc}
\toprule
Models & Total & Count & Relation & Depth & Distance
\\
\midrule
Qwen2-VL-2B & 31.38 & 54.69 & 22.46 & 0.16 & 31.66 \\
\midrule
~~$+$ SFT & 57.84 & 60.02 & 68.92 & 55.00 & 45.83 \\
~~$+$ GRPO & 59.47 & 59.64 & 66.76 & 54.16 & 56.66 \\
\rowcolor{mygray}~~$+$ GPG & 69.11 & 65.36 & 82.62 & 67.83 & 60.67 \\
% ~~$\Delta$ & \bf{+9.64} & \bf{+5.72} & \bf{+15.86} & \bf{+13.67} & \bf{+4.01} \\
\bottomrule
\end{tabular}
\caption{Visual reasoning results on CV-Bench~\cite{CV-Bench}, which shows GPG training on base model has overall better performance over GRPO training and the base model.}
\label{tab:CVBench}
\end{table}

==> ICLR26/tab/abaltion_dapo.tex <==
\begin{table}[h]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.5mm}
\small
% \resizebox{\textwidth}{!}{
  \begin{tabular}{cccccccccc}
    \toprule
    Method & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench & Training Cost & Data Cost & Memory \\
    \midrule
    DAPO-7B & 56.0& 30.0 & 84.6 & 82.5 & 34.9 &  47.8 & 1$\times$ & 1$\times$ & 28G\\
    \rowcolor{mygray}\ours-Zero-7B  & 57.7 & 36.7 & 84.6 &  82.5 & 39.0 &45.8 &  0.45$\times$ & 0.39$\times$ & 24G\\
    \bottomrule
  \end{tabular}
% }
\caption{Comparison with DAPO  (Qwen-7B Math). Ours is simpler, stronger and resource efficient.}
\label{tab:ablation_dapo}
\end{table}

==> ICLR26/tab/ablation_beta.tex <==
\begin{table}[h]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{1.8mm}
% \resizebox{\textwidth}{!}{
  \begin{tabular}{ccccccc}
    \toprule
    $\beta_{th}$ & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
    \midrule
    0.6& 48.3 & 30.0 & 76.2 & 62.5 & 34.2 & 39.0\\ 
    0.8 &48.6& 33.3 & 73.6& 67.5& 29.4& 39.3\\
    % \midrule
    % 2 & 41.9 & 23.3 & 70.0 & 57.5& 25.0 & 33.9\\
    % 4 & 42.5& 16.7 & 73.6 & 52.5 &30.1& 39.4\\
    % 8& 47.0&26.7& 75.8& 60.0 & 32.3 & 40.0\\
    % 16& 46.4 & 23.3 & 77.6 & 65.0 & 29.8 & 36.1 \\
    \bottomrule
  \end{tabular}
% }
\caption{Ablation on different $\beta_{th}$  using Qwen2.5 Math 7B.}
\label{tab:ablation_beta}
\end{table}

==> ICLR26/tab/ablation_ngen.tex <==
\begin{table}[h]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{1.8mm}
% \resizebox{\textwidth}{!}{
  \begin{tabular}{ccccccc}
    \toprule
    Group Number & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
    \midrule
    2& 41.9 & 16.7 & 71.6&60.0 &25.0& 36.0\\
    4& 43.3 & 20.0 & 73.2& 55.0 & 29.8& 38.5 \\ 
    8 & 45.3&23.3 & 73.6 & 60.0 & 30.5 & 39.3  \\
    16 &47.3& 26.7 & 74.6& 65.0& 32.4& 37.8\\
    % \midrule
    % 2 & 41.9 & 23.3 & 70.0 & 57.5& 25.0 & 33.9\\
    % 4 & 42.5& 16.7 & 73.6 & 52.5 &30.1& 39.4\\
    % 8& 47.0&26.7& 75.8& 60.0 & 32.3 & 40.0\\
    % 16& 46.4 & 23.3 & 77.6 & 65.0 & 29.8 & 36.1 \\
    \bottomrule
  \end{tabular}
% }
\caption{Ablation on different group size (wo AGE) using Qwen2.5 Math 7B.}
\label{tab:ablation_ngen}
\end{table}

==> ICLR26/tab/ablation_std_norm.tex <==
\begin{table}[h]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\adjustbox{max width=\textwidth}{
\setlength{\tabcolsep}{3pt}
  \begin{tabular}{ccccccc}
    \toprule
    $F_{norm}$& Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
    \midrule
    Group & 45.3&23.3 & 73.6 & 60.0 & 30.5 & 39.3  \\
    Batch & 44.9 & 23.3 & 72.2 & 55.0 & 35.3 & 38.5\\
    1 & 43.9 & 23.3 & 76.3 &52.5 & 30.1 & 37.4 \\
    % + KL ($\beta$=0.04) & 43.7 & 20.0 & 73.8 & 57.5 & 29.4 & 37.6\\
    % \rowcolor{mygray}Wo &47.0&26.7& 75.8& 60.0 & 32.3 & 40.0\\
    \bottomrule
  \end{tabular}
}
\caption{Ablation on reward normalization using Qwen2.5 Math 7B. }
\label{tab:ablation_std_norm}
\end{table}

==> ICLR26/tab/compare.tex <==
\begin{table}[!ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{4}{c}{Components} \\
\cmidrule(lr){2-5}
& Value Models & Reference Models & Surrogate Loss & Policy Constraint \\
\midrule
PPO  & \checkmark          & \checkmark          & \checkmark          & \checkmark          \\
GRPO & \ding{55}          & \checkmark          & \checkmark          & \checkmark          \\
TRPO & \checkmark          & \ding{55}          & \checkmark          & \checkmark          \\
% PG   & \checkmark          & $\times$          & $\times$          & $\times$          \\
\rowcolor{mygray}GPG & \ding{55}          & \ding{55}          & \ding{55}         & \ding{55}
\\
\bottomrule
\end{tabular}
\caption{Comparison of reinforcement learning algorithms (in reasoning) with various components.}
\label{tab:compare}
\end{table}

==> ICLR26/tab/math-all-15B.tex <==
\begin{table}[ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.4mm}
  \begin{tabular}{lcccccc}
    \toprule
    \textbf{Distilled 1.5B Models} & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench   \\
    % \midrule
    % \multicolumn{7}{l}{\textbf{General Models}} \\
    % Llama-3.1-70B-Instruct & 35.7 & 16.7 & 64.6 & 30.1 & 35.3 & 31.9   \\
    % o1-preview & \textbf{44.6} & 85.5 & - & - & - & -  \\
    \midrule
    % \multicolumn{7}{l}{\textbf{1.5B Models}} \\
    DeepSeek-R1-Distill-Qwen-1.5B & 48.9 & 28.8 & 82.8 & 62.9 & 26.5 & 43.3   \\
%     ~~+ GRPO & 53.1 & 33.3 & 83.8 & 67.5 & 29.8 & 50.9  \\
% \rowcolor{mygray}~~+ GPG & 55.7 & 33.3 & 87.6 & 77.5 & 29.4 & 50.5  \\
    % \midrule
    Still-3-1.5B-Preview & 51.6 & 32.5 & 84.4 & 66.7 & 29.0 & 45.4   \\
    % DeepScaleR-1.5B-Preview & \textbf{57.0} & \underline{43.1} & \textbf{87.8} & 73.6 & 30.2 & 50.0  \\
    Open-RS1$^\dagger$  & 53.1 & 33.3 & 83.8 & 67.5 & 29.8 & 50.9   \\
    % Open-RS2 (50 steps) & 30.0 & 85.4 & 80.0 & 30.5 & 52.4 & 55.7 \\
    Open-RS3$^\dagger$  & 52.0 & 26.7 & 85.4 & 70.0 & 27.9 & 50.2   \\
%     \midrule
% \rowcolor[HTML]{DAEFF9}\multicolumn{8}{l}{\textbf{Our Model}} \\
\rowcolor{mygray}\ours-RS1 & 55.7 & 33.3 &87.6 & 77.5 & 29.4 & 50.5  \\
\rowcolor{mygray}\ours-RS3 & 55.5 & 33.3 & 85.0 &80.0 & 26.8 & 52.4  \\
% \rowcolor{mygray}\ours-RS3 w/o STD norm &&&&&& \\
    \bottomrule
  \end{tabular}
\caption{The zero-shot pass@1 performance of the 1.5B models distilled by DeepSeek-R1 across five mathematical reasoning benchmarks. $\dagger$:  reproduced results using released codes. $\ddagger$: results from \citep{open-rs}.}
% }
\label{math-all-15B}
\end{table}

==> ICLR26/tab/math-all-7B.tex <==
\begin{table}[ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.4mm}
\resizebox{0.99\textwidth}{!}{
  \begin{tabular}{lcccccc}
    \toprule
    \textbf{7B Models} & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench   \\
    % o1-preview & \textbf{44.6} & 85.5 & - & - & - & -  \\
    \midrule
    % \multicolumn{7}{l}{\textbf{7B Models}} \\
    % \multicolumn{7}{l}{\textbf{7B Models}} \\
    Qwen-2.5-Math-7B-Instruct  $^\ddagger$ & 43.8& 13.3 & 79.8 & 50.6 & 34.6 & 40.7 \\
    Qwen2.5-Math-7B & 30.9 & 13.3 & 57.6 & 45.0 & 14.7 & 23.7 \\
    Qwen2.5-Math-7B (no template)$^\star$ & 38.2 & 0.2 & 69.0 & 45.8 & 21.3 & 34.7 \\
    rStar-Math-7B \citep{guan2025rstar}   &-& 26.7 & 78.4 & 47.5 & - & 47.1\\
    Eurus-2-7B-PRIME \citep{cui2025process} & 48.9 & 26.7 & 79.2 & 57.8 & 38.6 & 42.1\\
    Oat-Zero-7B \citep{liu2025understanding} & 51.4 & 43.3 & 80.0 & 62.7 & 30.1& 41.0 \\
    Oat-Zero-7B \citep{liu2025understanding}$^\dagger$  & 47.8 & 30.0 & 80.6 & 55.4 & 29.0 & 44.0 \\
    OpenReasoner-Zero-7B @ 8k \citep{hu2025open} & 45.9 & 13.3 &  82.4 &54.2  & 31.6 & 47.9 \\
    SimpleRL-Zero-7B \citep{zeng2025simplerl}$^\star$ &46.6  & 26.7 & 78.2 & 60.2 & 27.6 & 40.3\\
    \rowcolor{mygray}\ours-Zero-7B & 57.7 & 36.7  & 84.6  &  82.5  & 39.0   &45.8  \\
    % Qwen2.5-7B-SimpleRL & 26.7 & 82.4 & 62.5 & \textbf{39.7} & 43.3 & 50.9 & 864h \\
    \bottomrule
  \end{tabular}
  }
\caption{The zero-shot pass@1 performance of the 7B models across five mathematical reasoning benchmarks.
$\dagger$:  reproduced results using the released code. $\ddagger$: results from \citep{open-rs}, $^\star$: results from \citep{liu2025understanding}.}
% }
\label{math-all-7B}
\vspace{-0.2cm}
\end{table}

==> ICLR26/tab/mllm_tab_all.tex <==
\begin{table*}[!ht]
\begin{minipage}[ht]{0.34\textwidth}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.5cm}
% \captionsetup{skip=5pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc}
\toprule
Models & GEOQA$_{\text{Test}}$
\\
\midrule
Qwen2.5-VL-3B-Instruct & 35.41 \\
\midrule
~~$+$ GRPO & 47.48  \\
\rowcolor{mygray}~~$+$ GPG & 51.33  \\
% ~~$\Delta$ & \bf{+3.32} \\
\bottomrule
\end{tabular}
}
\caption{Geometry reasoning results on GEOQA. GPG is better than GRPO.}
\label{tab:GEOQA}
\end{minipage}
\hfill
\begin{minipage}[ht]{0.62\textwidth}
\centering
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc}
\toprule
Models & Average & Flower102~\cite{Flower102} & Pets37~\cite{Pets37} & FGVC~\cite{FGVCAircraft} & Cars196~\cite{Car196}
\\
\midrule
Qwen2-VL-2B  & 56.0 & 54.8 & 66.4 & 45.9 & 56.8 \\
\midrule
~~$+$ SFT & 55.6 & 58.5 & 55.5 & 67.9 & 40.5 \\
~~$+$ GRPO & 81.9 & 71.4 & 86.1 & 74.8 & 95.3 \\
\rowcolor{mygray}~~$+$ GPG & 89.0 & 79.3 & 90.8 & 88.5 & 97.5 \\
% ~~$\Delta$ & \bf{+4.1} & \bf{+1.6} & \bf{+1.0} & \bf{+12.0} & \bf{+1.8} \\
\bottomrule
\end{tabular}
}
\caption{4-shot Results on Four Fine-grained Classification Datasets. GPG shows consistently better results than GRPO on $4$ classification datasets.}
\label{tab:CLS}
\end{minipage}
\end{table*}

\begin{table*}[!ht]
\begin{minipage}[ht]{0.56\textwidth}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.5cm}
% \captionsetup{skip=5pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccc}
\toprule
Models & Total & Count & Relation & Depth & Distance
\\
\midrule
Qwen2-VL-2B & 31.38 & 54.69 & 22.46 & 0.16 & 31.66 \\
\midrule
~~$+$ SFT & 57.84 & 60.02 & 68.92 & 55.00 & 45.83 \\
~~$+$ GRPO & 59.47 & 59.64 & 66.76 & 54.16 & 56.66 \\
\rowcolor{mygray}~~$+$ GPG & 76.15 & 66.62 & 83.23 & 81.66 & 75.50 \\
% ~~$\Delta$ & \bf{+9.64} & \bf{+5.72} & \bf{+15.86} & \bf{+13.67} & \bf{+4.01} \\
\bottomrule
\end{tabular}
}
\caption{Visual reasoning results on CV-Bench~\citep{CV-Bench}, which shows GPG training on base model has overall better performance over GRPO and the base model.}
\label{tab:CVBench}
\end{minipage}
\hfill
\begin{minipage}[ht]{0.40\textwidth}
\centering
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Models & mIoU$_{\text{test}}$ & mIoU$_{\text{val}}$ & gIoU$_{\text{test}}$
\\
\midrule
Qwen2-VL-2B & 26.9 & 30.1 & 25.3 \\
\midrule
~~$+$ SFT & 28.3 & 29.7 & 25.3 \\
~~$+$ GRPO & 37.6 & 34.4 & 34.4 \\
\rowcolor{mygray}~~$+$ GPG & 51.8 & 51.3 & 50.4 \\
% ~~$\Delta$ & \bf{+13.9} & \bf{+19.0} & \bf{+15.1}\\
\bottomrule
\end{tabular}
}
\caption{Reasoning grounding results on LISA~\citep{LISA}. GPG surpasses GRPO in reasoning grounding.}
\label{tab:LISA}
\end{minipage}
\end{table*}

==> ICLR26/tab/open-r1.tex <==
\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{0.4mm}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.5cm}
% \captionsetup{skip=5pt}
  \begin{tabular}{lcccccc}
    \toprule
    Models & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
    \midrule
    Qwen2.5-Math-7B & 30.9 & 13.3 & 57.6 & 45.0 & 14.7 & 23.7 \\
    \midrule
    GPRO & 43.7 & 16.7 & 73.4 & 62.5 & 30.2 & 35.7  \\
% \ours($F_{norm}$=1,$\alpha$=1) & 43.9 & 23.3 & 76.3 &52.5 & 30.1 & 37.4 \\
\ours($F_{norm}$=1,$\alpha$=1) & 43.9 & 23.3 & 76.3 &52.5 & 30.1 & 37.4 \\
\ours($F_{norm}$=${\operatorname{std}\{R(o)\}}$,$\alpha$=1) & 45.3 & 23.3 & 73.6 & 60.0 & 30.5 & 39.3 \\
\ours($F_{norm}$=${\operatorname{std}\{R(o)\}}$,$\alpha=\frac{B}{B-M}$) & 44.1 & 23.3 & 74.2 & 52.5 & 30.9 & 39.7 \\
\rowcolor{mygray}\ours($F_{norm}$=1, $\alpha=\frac{B}{B-M}$) & 47.8 & 30.0 & 75.0 & 62.5& 33.1 & 38.2\\
\rowcolor{mygray}\ours ($F_{norm}$=1, $\alpha=\frac{B}{B-M}, \beta_{th}=0.6$) & 48.3 & 30.0 & 76.2 & 62.5 & 34.2 & 39.0\\

\midrule
   Dr. GRPO$^\dagger$ & 43.7 & 26.7&74.6&50.0&30.1&37.3\\

% \rowcolor{mygray}~~+ GPG w/o STD norm &47.0&26.7& 75.8& 60.0 & 32.3 & 40.0\\
% ~~$\Delta$ & \bf{+1.6} & \bf{+6.6} & \bf{+0.2} & -2.5 & \bf{+0.3} & \bf{+3.6} \\
    \bottomrule
  \end{tabular}
  \caption{Math reasoning results on Qwen2.5-Math-7B model. $\dagger$: reproduction use the released code.}
  \vspace{3mm}
  \label{tab:open-r1}
\end{table}

==> ICLR26/tab/open-rs-15B.tex <==
% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{1.4mm}
% \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{-0.3cm}
% % \captionsetup{skip=5pt}
%   \begin{tabular}{lcccccc}
%     \toprule
%     Models & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
%     \midrule
%     Base Model & 48.9 & 28.8 & 82.8 & 62.9 & 26.5 & 43.3 \\
%     \midrule
% ~~+ GRPO & 52.0 & 26.7 & 85.4 & 70.0 & 27.9 & 50.2  \\
% \rowcolor{mygray}~~+ GPG & 55.5 & 33.3 & 85.0 & 80.0 & 26.8 & 52.4  \\
% % \rowcolor{mygray}~~+ GPG w/o STD norm & & & & & & \\
% % ~~$\Delta$ & \bf{+2.6} & +0.0 & \bf{+3.8} & \bf{+10.0} & -0.4 & -0.4 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Results on the DeepSeek-R1-Distill-Qwen-1.5B model. GPG method achieved an additional average performance boost of 3.5\% compared to GRPO.}
%   \label{tab:open-rs}
% \end{table}

\begin{table}[ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
\captionsetup{skip=5pt}
  \begin{tabular}{lcccccc}
    \toprule
    Models & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench  \\
    \midrule
    Base Model & 48.9 & 28.8 & 82.8 & 62.9 & 26.5 & 43.3 \\
    \midrule
% ~~+ GRPO & 53.1 & 33.3 & 83.8 & 67.5 & 29.8 & 50.9  \\
% \rowcolor{mygray}~~+ GPG & 55.7 & 33.3 & 87.6 & 77.5 & 29.4 & 50.5  \\
% ~~$\Delta$ & \bf{+2.6} & +0.0 & \bf{+3.8} & \bf{+10.0} & -0.4 & -0.4 \\
    \bottomrule
  \end{tabular}
  \caption{Results on the DeepSeek-R1-Distill-Qwen-1.5B model. GPG method achieved an additional average performance boost of 2.6\% compared to GRPO.}
  \label{tab:open-rs}
\end{table}

==> ICLR26/tab/open-rs-all.tex <==
\begin{table}[ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.4mm}
  \begin{tabular}{lcccccc}
    \toprule
    Model & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench   \\
    \midrule
    \multicolumn{7}{l}{\textbf{General Models}} \\
    Llama-3.1-70B-Instruct & 35.7 & 16.7 & 64.6 & 30.1 & 35.3 & 31.9   \\
    % o1-preview & \textbf{44.6} & 85.5 & - & - & - & -  \\
    \midrule
    % \multicolumn{7}{l}{\textbf{7B Models}} \\
    Qwen-2.5-Math-7B-Instruct \cite{yang2024qwen25mathtechnicalreportmathematical} $^\ddagger$ & 43.8& 13.3 & 79.8 & 50.6 & 34.6 & 40.7 \\
    Qwen2.5-Math-7B & 30.9 & 13.3 & 57.6 & 45.0 & 14.7 & 23.7 \\
    rStar-Math-7B \cite{guan2025rstar}   &-& 26.7 & 78.4 & 47.5 & - & 47.1\\
    Eurus-2-7B-PRIME \cite{cui2025process} & 48.9 & 26.7 & 79.2 & 57.8 & 38.6 & 42.1\\
    Oat-Zero-7B \cite{liu2025understanding} & 51.4 & 43.3 & 80.0 & 62.7 & 30.1& 41.0 \\
    Oat-Zero-7B$^\dagger$  & 47.8 & 30.0 & 80.6 & 55.4 & 29.0 & 44.0 \\
    OpenReasoner-Zero-7B @ 8k \cite{hu2025open} & 45.9 & 13.3 &  82.4 &54.2  & 31.6 & 47.9 \\
    SimpleRL-Zero-7B \cite{zeng2025simplerl} &46.6  & 26.7 & 78.2 & 60.2 & 27.6 & 40.3\\
    \ours-7B & & \\

    % Qwen2.5-7B-SimpleRL & 26.7 & 82.4 & 62.5 & \textbf{39.7} & 43.3 & 50.9 & 864h \\
    \midrule
    \multicolumn{7}{l}{\textbf{1.5B Models}} \\
    DeepSeek-R1-Distill-Qwen-1.5B & 48.9 & 28.8 & 82.8 & 62.9 & 26.5 & 43.3   \\
    Still-3-1.5B-Preview & 51.6 & 32.5 & 84.4 & 66.7 & 29.0 & 45.4   \\
    % DeepScaleR-1.5B-Preview & \textbf{57.0} & \underline{43.1} & \textbf{87.8} & 73.6 & 30.2 & 50.0  \\
    Open-RS1$^\dagger$  & 53.1 & 33.3 & 83.8 & 67.5 & 29.8 & 50.9   \\
    % Open-RS2 (50 steps) & 30.0 & 85.4 & 80.0 & 30.5 & 52.4 & 55.7 \\
    Open-RS3$^\dagger$  & 52.0 & 26.7 & 85.4 & 70.0 & 27.9 & 50.2   \\
%     \midrule
% \rowcolor[HTML]{DAEFF9}\multicolumn{8}{l}{\textbf{Our Model}} \\
\rowcolor{mygray}\ours-RS1 & 55.7 & 33.3 &87.6 & 77.5 & 29.4 & 50.5  \\
\rowcolor{mygray}\ours-RS3 & 55.5 & 33.3 & 85.0 &80.0 & 26.8 & 52.4  \\
% \rowcolor{mygray}\ours-RS3 w/o STD norm &&&&&& \\
    \bottomrule
  \end{tabular}
\caption{Zero-shot pass@1 performance across benchmarks. $\dagger$:  reproduced results using the released code. $\ddagger$: results from \cite{open-rs}.}
% }
\label{open-rs-all}
\end{table}

==> iclr_rebuttal_code_result_tab.tex <==
\begin{table}[htbp]
\centering
\caption{EvalPlus Code Result}
\label{tab:evalplus_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cc|cc|}
\hline
\multirow{2}{*}{\textbf{model}} & \multicolumn{2}{c|}{\textbf{HumanEval}} & \multicolumn{2}{c|}{\textbf{MBPP}} \\
\cline{2-5}
 & Base & Plus & Base & Plus \\
\hline
% deepseek-ai/DeepSeek-R1-Distill-Qwen-1.5B & 40.24\% & 37.20\% & 25.13\% & 22.49\% \\
GRPO & 38.41\% & 34.76\% & 24.60\% & 21.96\% \\
GPG & 37.80\% & 34.15\% & 26.19\% & 23.81\% \\
\hline
\end{tabular}
}
\end{table}


==> iclr_rebuttal_qa_result_tab.tex <==
\begin{table}[htbp]
\centering
\caption{Zero Shot evaluation results based on Light-eval. }
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|cccc|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Seed} & \multicolumn{4}{c|}{arc\string:challenge} & \multicolumn{4}{c|}{arc\string:easy} & \multicolumn{4}{c|}{hellaswag} & \multicolumn{4}{c|}{truthfulqa\string:mc} \\
 &  & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & acc & acc\_stderr & acc\_norm & acc\_norm\_stderr & mc1 & mc1\_stderr & mc2 & mc2\_stderr \\
\hline
% \multirow{4}{*}{DeepSeek-R1-Distill-Qwen-1.5B} & 0 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 1 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 2 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
%  & 3 & 26.962 & 1.297 & 30.034 & 1.340 & 38.468 & 0.998 & 35.059 & 0.979 & 36.188 & 0.480 & 42.541 & 0.493 & 35.006 & 1.670 & 50.160 & 1.535 \\
% \hline
\multirow{4}{*}{GRPO} & 0 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 1 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 2 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
 & 3 & 30.205 & 1.342 & 33.191 & 1.376 & 43.392 & 1.017 & 36.322 & 0.987 & 36.248 & 0.480 & 41.914 & 0.492 & 29.376 & 1.595 & 47.307 & 1.516 \\
\hline
\multirow{4}{*}{GPG} & 0 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 1 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 2 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
 & 3 & 27.048 & 1.298 & 30.375 & 1.344 & 38.721 & 1.000 & 35.311 & 0.981 & 36.118 & 0.479 & 42.551 & 0.493 & 34.884 & 1.668 & 50.146 & 1.533 \\
\hline
\end{tabular}
}% end resizebox
\end{table}

==> sec/6_reproducibility.tex <==
\section{Reproducibility Statement}
We have taken the following steps to ensure the reproducibility of our empirical results:
(1) We provide a comprehensive description of all experimental setups, including the datasets used and their corresponding benchmarks, in Section \ref{Section3.1}.
(2) Our implementation builds upon several publicly available code repositories. For unimodal tasks, we utilize the VERL framework \citep{sheng2024hybridflow}, Open-r1 \citep{open-r1}, and Open-rs \citep{open-rs}. For multimodal tasks, we adopt VisualThinker-R1-Zero \citep{VisualThinker-R1-Zero}, R1-V \citep{R1-V}, and Visual-RFT \citep{Visual-RFT}. These repositories have been adapted to suit our purposes and to facilitate replication by the research community.
(3) Detailed training configurations—including hyperparameters, evaluation protocols, and specific adaptations applied to each base framework—are thoroughly documented in Appendices \ref{sec:detailed setting}.
(4) In compliance with the double-blind review policy, we have made our full implementation, along with training and evaluation scripts, publicly accessible through an anonymous repository. This ensures that all reported results can be reproduced without revealing the authors’ identities.

==> tab/C-EVAL.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|c|c|c}
        \hline
        \textbf{C-Eval Datasets} & \textbf{Deepseek-R1-Distill-Qwen-1.5B} & \textbf{GPG} & \textbf{Accuracy Gain} \\ \hline
        computer network & 9.09 & 9.09 & 0.00 \\ 
        operating system & 42.86 & 43.36 & +0.50 \\ 
        computer architecture & 28.57 & 27.93 & -0.64 \\ 
        college programming & 50.00 & 50.00 & 0.00 \\ 
        college physics & 16.67 & 17.49 & +0.82 \\ 
        college chemistry & 42.86 & 42.86 & 0.00 \\ 
        advanced mathematics & 42.11 & 41.83 & -0.28 \\ 
        probability and statistics & 38.89 & 39.30 & +0.41 \\ 
        discrete mathematics & 20.57 & 21.05 & +0.48 \\ 
        electrical engineer & 38.89 & 38.89 & 0.00 \\ 
        metrology engineer & 12.00 & 13.40 & +1.40 \\ 
        high school mathematics & 20.78 & 21.67 & +0.89 \\ 
        high school physics & 47.18 & 50.67 & +3.49 \\ 
        high school chemistry & 49.00 & 50.25 & +1.25 \\ 
        high school biology & 22.22 & 22.54 & +0.32 \\ 
        middle school mathematics & 26.67 & 26.34 & -0.33 \\ 
        middle school biology & 39.00 & 38.37 & -0.63 \\ 
        middle school physics & 42.86 & 45.93 & +3.07 \\ 
        middle school chemistry & 33.33 & 32.47 & -0.86 \\ 
        veterinary medicine & 46.15 & 47.13 & +0.98 \\ 
        college economics & 57.89 & 57.89 & 0.00 \\ 
        business administration & 15.38 & 19.88 & +4.50 \\ 
        marxism & 30.82 & 30.82 & +0.00 \\ 
        mao zedong thought & 16.67 & 17.06 & +0.39 \\ 
        education science & 45.45 & 45.16 & -0.29 \\ 
        teacher qualification & 55.56 & 57.68 & +2.12 \\ 
        high school politics & 21.43 & 29.24 & +7.81 \\ 
        high school geography & 27.27 & 28.11 & +0.84 \\ 
        middle school politics & 29.56 & 29.56 & 0.00 \\ 
        middle school geography & 4.73 & 4.73 & 0.00 \\ 
        modern chinese history & 25.00 & 25.00 & 0.00 \\ 
        ideological and moral cultivation & 39.98 & 39.98 & 0.00 \\ 
        logic & 46.67 & 46.02 & -0.65 \\ 
        law & 26.67 & 20.33 & -6.34 \\ 
        chinese language and literature & 15.38 & 14.79 & -0.59 \\ 
        art studies & 35.71 & 35.71 & 0.00 \\ 
        professional tour guide & 20.00 & 20.00 & 0.00 \\ 
        legal professional & 7.14 & 6.66 & -0.48 \\ 
        high school chinese & 41.67 & 41.67 & 0.00 \\ 
        high school history & 41.67 & 42.21 & +0.54 \\ 
        middle school history & 9.09 & 9.09 & 0.00 \\ 
        civil servant & 47.37 & 47.84 & +0.47 \\ 
        sports science & 62.48 & 62.48 & 0.00 \\ 
        plant protection & 33.33 & 34.33 & +1.00 \\ 
        basic medicine & 44.44 & 43.74 & -0.70 \\ 
        clinical medicine & 42.86 & 42.16 & -0.70 \\ 
        urban and rural planner & 57.14 & 61.44 & +4.30 \\ 
        accountant & 23.53 & 22.77 & -0.76 \\ 
        fire engineer & 41.67 & 41.67 & 0.00 \\ 
        environmental impact engineer & 19.05 & 18.34 & -0.71 \\ 
        tax accountant & 30.75 & 29.22 & -1.53 \\ 
        physician & 25.00 & 24.79 & -0.21 \\ 
        \rowcolor{mygray} \textbf{AVERAGE} & \textbf{32.91} & \textbf{33.29} & \textbf{+0.38} \\ \hline
    \end{tabular}
    \caption{Comparison of performance metrics across general C-Eval datasets.}
    \vspace{-5mm}
    \label{tab:ceval}
\end{table}

==> tab/GEOQA-LISA-merge.tex <==
\begin{table*}[!ht]
\begin{minipage}[ht]{0.44\textwidth}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.5cm}
% \captionsetup{skip=5pt}
\centering
\begin{tabular}{lc}
\toprule
Models & GEOQA$_{\text{Test}}$
\\
\midrule
Qwen2.5-VL-3B-Instruct & 35.41 \\
\midrule
~~$+$ GRPO & 47.48  \\
\rowcolor{mygray}~~$+$ GPG & 50.80  \\
% ~~$\Delta$ & \bf{+3.32} \\
\bottomrule
\end{tabular}
\caption{Geometry reasoning results on GEOQA~\cite{GEOQA}. GPG is better than GRPO.}
\label{tab:GEOQA}
\end{minipage}
\hfill
\begin{minipage}[ht]{0.52\textwidth}
\centering
\begin{tabular}{lccc}
\toprule
Models & mIoU$_{\text{test}}$ & mIoU$_{\text{val}}$ & gIoU$_{\text{test}}$
\\
\midrule
Qwen2-VL-2B & 26.9 & 30.1 & 25.3 \\
\midrule
~~$+$ SFT & 28.3 & 29.7 & 25.3 \\
~~$+$ GRPO & 37.6 & 34.4 & 34.4 \\
\rowcolor{mygray}~~$+$ GPG & 51.5 & 53.4 & 49.5 \\
% ~~$\Delta$ & \bf{+13.9} & \bf{+19.0} & \bf{+15.1}\\
\bottomrule
\end{tabular}
\caption{Reasoning grounding results on LISA~\cite{LISA}. GPG surpasses GRPO in reasoning grounding with 239 training images.}
\label{tab:LISA}
\end{minipage}
\end{table*}

==> tab/MMLU.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{l|c|c|c}
        \hline
        \textbf{MMLU Datasets} & \textbf{Deepseek-R1-Distill-Qwen-1.5B} & \textbf{+GPG} & \textbf{Accuracy Gain} \\ \hline
        college biology & 24.31 & 24.31 & 0.00 \\ 
        college chemistry & 32.00 & 32.00 & 0.00 \\ 
        college computer science & 21.00 & 21.00 & 0.00 \\ 
        college mathematics & 32.00 & 32.00 & 0.00 \\ 
        college physics & 28.43 & 30.39 & +1.96 \\ 
        electrical engineering & 50.34 & 50.34 & 0.00 \\ 
        astronomy & 36.84 & 38.16 & +1.32 \\ 
        anatomy & 35.56 & 35.56 & 0.00 \\ 
        abstract algebra & 27.00 & 27.00 & 0.00 \\ 
        machine learning & 37.50 & 37.50 & 0.00 \\ 
        clinical knowledge & 41.89 & 42.64 & +0.75 \\ 
        global facts & 31.00 & 30.00 & -1.00 \\ 
        management & 43.69 & 43.69 & 0.00 \\ 
        nutrition & 38.89 & 38.89 & 0.00 \\ 
        marketing & 58.55 & 58.55 & 0.00 \\ 
        professional accounting & 29.08 & 28.72 & -0.36 \\ 
        high school geography & 44.95 & 45.45 & +0.50 \\ 
        international law & 45.45 & 47.11 & +1.66 \\ 
        moral scenarios & 24.13 & 24.36 & +0.23 \\ 
        computer security & 39.00 & 39.00 & 0.00 \\ 
        high school microeconomics & 44.96 & 46.22 & +1.26 \\ 
        professional law & 27.71 & 28.16 & +0.45 \\ 
        medical genetics & 46.00 & 46.00 & 0.00 \\ 
        professional psychology & 33.5 & 33.66 & +0.16 \\ 
        jurisprudence & 39.81 & 39.81 & 0.00 \\ 
        world religions & 33.92 & 33.33 & -0.59 \\ 
        philosophy & 41.48 & 42.12 & +0.64 \\ 
        virology & 40.96 & 40.96 & 0.00 \\ 
        high school chemistry & 38.42 & 39.41 & +0.99 \\ 
        public relations & 42.73 & 42.73 & 0.00 \\ 
        high school macroeconomics & 42.82 & 43.08 & +0.26 \\ 
        human sexuality & 48.85 & 48.85 & 0.00 \\ 
        elementary mathematics & 37.57 & 38.10 & +0.53 \\ 
        high school physics & 24.50 & 23.84 & -0.66 \\ 
        high school computer science & 42.00 & 42.00 & 0.00 \\ 
        high school european history & 40.00 & 40.61 & +0.61 \\ 
        business ethics & 43.00 & 43.00 & 0.00 \\ 
        moral disputes & 37.57 & 37.28 & -0.29 \\ 
        high school statistics & 50.00 & 50.46 & +0.46 \\ 
        miscellaneous & 44.32 & 44.57 & +0.25 \\ 
        formal logic & 29.37 & 29.37 & 0.00 \\ 
        high school government and politics & 38.34 & 38.86 & +0.52 \\ 
        prehistory & 32.72 & 33.33 & +0.61 \\ 
        security studies & 43.67 & 43.67 & 0.00 \\ 
        high school biology & 44.52 & 44.19 & -0.33 \\ 
        logical fallacies & 38.04 & 38.04 & 0.00 \\ 
        high school world history & 42.62 & 43.04 & +0.42 \\ 
        professional medicine & 38.60 & 38.97 & +0.37 \\ 
        high school mathematics & 30.00 & 30.74 & +0.74 \\ 
        college medicine & 32.37 & 32.95 & +0.58 \\ 
        high school us history & 35.78 & 35.78 & 0.00 \\ 
        sociology & 47.76 & 48.26 & +0.50 \\ 
        econometrics & 32.46 & 32.46 & 0.00 \\ 
        high school psychology & 42.94 & 42.75 & -0.19 \\ 
        human aging & 36.32 & 36.32 & 0.00 \\ 
        us foreign policy & 56.00 & 57.00 & +1.00 \\ 
        conceptual physics & 40.43 & 39.57 & -0.86 \\ 
        \rowcolor{mygray} \textbf{AVERAGE} & \textbf{38.31} & \textbf{38.53} & \textbf{+0.22} \\ \hline
    \end{tabular}
    }
    \caption{Comparison of performance metrics across general MMLU datasets.}
    \label{tab:mmlu}
    \vspace{-5mm}
\end{table}

==> tab/MMLU_Ceval.tex <==
\begin{table}[ht]
\centering
\label{tab:gpg_mmlu_ceval}
\setlength{\tabcolsep}{8mm}
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{MMLU} & \textbf{C-Eval} \\
\midrule
DeepSeek-R1-distill-qwen-1.5B & 38.31 & 32.91 \\
+ GPG                         & 38.53 (+0.22) & 33.29 (+0.38) \\
\bottomrule
\end{tabular}
\caption{Evaluation of GPG on MMLU and C-Eval.}
\end{table}


==> tab/Visual-RFT-CLS.tex <==
\begin{table}[!ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|c|cccc}
\toprule
Models & Average & Flower102~\cite{Flower102} & Pets37~\cite{Pets37} & FGVC~\cite{FGVCAircraft} & Cars196~\cite{Car196}
\\
\midrule
Qwen2-VL-2B  & 56.0 & 54.8 & 66.4 & 45.9 & 56.8 \\
\midrule
~~$+$ SFT & 55.6 & 58.5 & 55.5 & 67.9 & 40.5 \\
~~$+$ GRPO & 81.9 & 71.4 & 86.1 & 74.8 & 95.3 \\
\rowcolor{mygray}~~$+$ GPG & 86.0 & 73.0 & 87.1 & 86.8 & 97.1 \\
% ~~$\Delta$ & \bf{+4.1} & \bf{+1.6} & \bf{+1.0} & \bf{+12.0} & \bf{+1.8} \\
\bottomrule
\end{tabular}
\caption{4-shot Results on Four Fine-grained Classification Datasets. GPG shows consistently better results than GRPO on $4$ classification datasets.}
\label{tab:CLS}
\end{table}

==> tab/VisualThinker-R1-Zero-CV-Bench.tex <==
\begin{table}[!ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\begin{tabular}{l|c|cccc}
\toprule
Models & Total & Count & Relation & Depth & Distance
\\
\midrule
Qwen2-VL-2B & 31.38 & 54.69 & 22.46 & 0.16 & 31.66 \\
\midrule
~~$+$ SFT & 57.84 & 60.02 & 68.92 & 55.00 & 45.83 \\
~~$+$ GRPO & 59.47 & 59.64 & 66.76 & 54.16 & 56.66 \\
\rowcolor{mygray}~~$+$ GPG & 69.11 & 65.36 & 82.62 & 67.83 & 60.67 \\
% ~~$\Delta$ & \bf{+9.64} & \bf{+5.72} & \bf{+15.86} & \bf{+13.67} & \bf{+4.01} \\
\bottomrule
\end{tabular}
\caption{Visual reasoning results on CV-Bench~\cite{CV-Bench}, which shows GPG training on base model has overall better performance over GRPO training and the base model.}
\label{tab:CVBench}
\end{table}

==> tab/open-rs-all.tex <==
\begin{table}[ht]
\centering
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.1cm}
% \captionsetup{skip=5pt}
\setlength{\tabcolsep}{0.4mm}
  \begin{tabular}{lcccccc}
    \toprule
    Model & Average & AIME24 & MATH-500 & AMC23 & Minerva & OlympiadBench   \\
    \midrule
    \multicolumn{7}{l}{\textbf{General Models}} \\
    Llama-3.1-70B-Instruct & 35.7 & 16.7 & 64.6 & 30.1 & 35.3 & 31.9   \\
    % o1-preview & \textbf{44.6} & 85.5 & - & - & - & -  \\
    \midrule
    % \multicolumn{7}{l}{\textbf{7B Models}} \\
    Qwen-2.5-Math-7B-Instruct \cite{yang2024qwen25mathtechnicalreportmathematical} $^\ddagger$ & 43.8& 13.3 & 79.8 & 50.6 & 34.6 & 40.7 \\
    Qwen2.5-Math-7B & 30.9 & 13.3 & 57.6 & 45.0 & 14.7 & 23.7 \\
    rStar-Math-7B \cite{guan2025rstar}   &-& 26.7 & 78.4 & 47.5 & - & 47.1\\
    Eurus-2-7B-PRIME \cite{cui2025process} & 48.9 & 26.7 & 79.2 & 57.8 & 38.6 & 42.1\\
    Oat-Zero-7B \cite{liu2025understanding} & 51.4 & 43.3 & 80.0 & 62.7 & 30.1& 41.0 \\
    Oat-Zero-7B$^\dagger$  & 47.8 & 30.0 & 80.6 & 55.4 & 29.0 & 44.0 \\
    OpenReasoner-Zero-7B @ 8k \cite{hu2025open} & 45.9 & 13.3 &  82.4 &54.2  & 31.6 & 47.9 \\
    SimpleRL-Zero-7B \cite{zeng2025simplerl} &46.6  & 26.7 & 78.2 & 60.2 & 27.6 & 40.3\\
    \ours-7B & & \\

    % Qwen2.5-7B-SimpleRL & 26.7 & 82.4 & 62.5 & \textbf{39.7} & 43.3 & 50.9 & 864h \\
    \midrule
    \multicolumn{7}{l}{\textbf{1.5B Models}} \\
    DeepSeek-R1-Distill-Qwen-1.5B & 48.9 & 28.8 & 82.8 & 62.9 & 26.5 & 43.3   \\
    Still-3-1.5B-Preview & 51.6 & 32.5 & 84.4 & 66.7 & 29.0 & 45.4   \\
    % DeepScaleR-1.5B-Preview & \textbf{57.0} & \underline{43.1} & \textbf{87.8} & 73.6 & 30.2 & 50.0  \\
    Open-RS1$^\dagger$  & 53.1 & 33.3 & 83.8 & 67.5 & 29.8 & 50.9   \\
    % Open-RS2 (50 steps) & 30.0 & 85.4 & 80.0 & 30.5 & 52.4 & 55.7 \\
    Open-RS3$^\dagger$  & 52.0 & 26.7 & 85.4 & 70.0 & 27.9 & 50.2   \\
%     \midrule
% \rowcolor[HTML]{DAEFF9}\multicolumn{8}{l}{\textbf{Our Model}} \\
\rowcolor{mygray}\ours-RS1 & 55.7 & 33.3 &87.6 & 77.5 & 29.4 & 50.5  \\
\rowcolor{mygray}\ours-RS3 & 55.5 & 33.3 & 85.0 &80.0 & 26.8 & 52.4  \\
% \rowcolor{mygray}\ours-RS3 w/o STD norm &&&&&& \\
    \bottomrule
  \end{tabular}
\caption{Zero-shot pass@1 performance across benchmarks. $\dagger$:  reproduced results using the released code. $\ddagger$: results from \cite{open-rs}.}
% }
\label{open-rs-all}
\end{table}
